Let Go of Your Labels with Unsupervised Transfer

Foundation vision-language models have enabled remarkable zero-shot transferability of the pre-trained representations to a wide range of downstream tasks. However, to solve a new task, zero-shot transfer still necessitates human guidance to define visual categories that appear in the data. Here, we show that fully unsupervised transfer emerges when searching for the labeling of a dataset that induces maximal margin classifiers in representation spaces of different foundation models. We present TURTLE, a fully unsupervised method that effectively employs this guiding principle to uncover the underlying labeling of a downstream dataset without any supervision and task-specific representation learning. We evaluate TURTLE on a diverse benchmark suite of 26 datasets and show that it achieves new state-of-the-art unsupervised performance. Furthermore, TURTLE, although being fully unsupervised, outperforms zero-shot transfer baselines on a wide range of datasets. In particular, TURTLE matches the average performance of CLIP zero-shot on 26 datasets by employing the same representation space, spanning a wide range of architectures and model sizes. By guiding the search for the underlying labeling using the representation spaces of two foundation models, TURTLE surpasses zero-shot transfer and unsupervised prompt tuning baselines, demonstrating the surprising power and effectiveness of unsupervised transfer.

==> section/7limitations.tex <==
\section{Limitations}\label{limitations}
\xhdr{Number of classes and empirical label distribution} Following previous works on unsupervised learning \cite{van2020scan, niu2021spice, gadetsky2023pursuit}, \methodnew also assumes that samples of a downstream dataset are evenly distributed across $C$ classes, where $C$ is known a priori. However, the proposed framework is compatible with approaches which can estimate the required quantities from data \cite{fu2020estimating, mazumder2023deepvat}.

\xhdr{Applicability beyond vision domain} Although, in this work, we evaluate \methodnew solely on vision datasets, our framework is model-agnostic, \textit{i.e.}, it is compatible with any pre-trained representations. Therefore, \methodnew is applicable to other domains by taking advantage of unceasing progress in the development of foundation models for different data modalities \cite{elizade2022clap, elizade2023natural, lin2023pmc, robinson2023contrasting, meidani2024snip}.
